The Art of Optimizing T-Depth for Quantum Error Correction in Large-Scale Quantum Computing

Quantum Error Correction (QEC), combined with magic state distillation, ensures fault tolerance in large-scale quantum computation. To apply QEC, a circuit must first be transformed into a non-Clifford (or T) gate set. T-depth, the number of sequential T-gate layers, determines the magic state cost, impacting both spatial and temporal overhead. Minimizing T-depth is crucial for optimizing resource efficiency in fault-tolerant quantum computing. While QEC scalability has been widely studied, T-depth reduction remains an overlooked challenge. We establish that T-depth reduction is an NP-hard problem and systematically evaluate multiple approximation techniques: greedy, divide-and-conquer, Lookahead-based brute force, and graph-based. The Lookahead-based brute-force algorithm (partition size 4) performs best, optimizing 90\% of reducible cases (i.e., circuits where at least one algorithm achieved optimization) with an average T-depth reduction of around 51\%. Additionally, we introduce an expansion factor-based identity gate insertion strategy, leveraging controlled redundancy to achieve deeper reductions in circuits initially classified as non-reducible. With this approach, we successfully convert up to 25\% of non-reducible circuits into reducible ones, while achieving an additional average reduction of up to 11.8\%. Furthermore, we analyze the impact of different expansion factor values and explore how varying the partition size in the Lookahead-based brute-force algorithm influences the quality of T-depth reduction.

==> 2_circuit_gen.tex <==
\section{Generating Diverse Circuits} \label{sec:circuit_gen}

\textbf{Generation of Circuit Parameters:}
Our dataset spans 2,250 quantum circuits by varying qubits (10–100, 10 values), columns (15 values, 1 to $10 \times$ qubits), and T gates (15 values, $\max(\text{qubits}, \text{columns})$ to qubits $\times$ columns). Scaling columns up to $100 \times$ qubits ensures coverage of both shallow, high-parallelism and deep, high-depth circuits.
\textbf{Structured Circuit Construction:}
A random circuit generator simulates quantum circuits as a 2D array, where rows represent qubits and columns define depth. Each circuit is parameterized by qubits, columns, and T gates, which are randomly placed while ensuring each qubit and column contains at least one. Columns are assigned a random phase (`$+$' or `$-$'), and all gates initially default to identity (`I'). The remaining T gates are uniformly distributed, preserving a balanced structure.
\textbf{Circuit Size-Based Classification:}
We classify circuits using a three-layer framework based on depth, T-gate density, and qubit system size, yielding 27 categories ($3 \times 3 \times 3$). Depth is determined by column count percentiles: Shallow (S), Medium (M), and Deep (D). T-gate density, defined as $T_{\text{Gate Density}} = \frac{\text{Total T Gates}}{\text{Qubits} \times \text{Columns}}$, is categorized as Low (L), Medium (M), or High (H). Qubit system size is classified as Small (S), Medium (M), or Large (L). Circuits are labeled DTQ (Depth-T-Gate-Qubit), e.g., S-L-S for \underline{S}hallow, \underline{L}ow T-Gate Density, \underline{S}mall Qubit system, or D-H-L for \underline{D}eep, \underline{H}igh T-Gate Density, \underline{L}arge Qubit system.


==> extra.tex <==
\begin{table*}[]
\centering
\caption{Results of Algorithmic and Optimization Strategies across Various Circuit Categories and Subcategories}
\begin{adjustbox}{angle=90}
% \vspace{-100pt}
\fontsize{9.5pt}{10.5pt}\selectfont
\begin{tabular}{ccc||cc||ccc||ccccc}
\hline \hline
\multicolumn{3}{c||}{\textbf{Classification}}                                                                                                                                             & \multicolumn{2}{c||}{\textbf{Algorithm}}                              & \multicolumn{3}{c||}{\textbf{Original Circuit}} & \multicolumn{5}{c}{\textbf{Optimized Results}}                                                                             \\ \hline
\multicolumn{1}{c||}{\textbf{Category}}                                                                   & \multicolumn{1}{c|}{\textbf{Sub Cat.}}                 & \textbf{Class}       & \multicolumn{1}{c|}{\textbf{Type}}           & \textbf{Optimization} & \textbf{\#Q}   & \textbf{\#C}  & \textbf{\#T}  & \textbf{Data Block} & \textbf{Protocols}                           & \textbf{\#Steps} & \textbf{\#Idle} & \textbf{\#Tiles} \\ \hline \hline
\multicolumn{1}{c|}{\multirow{16}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Circuit\\ Depth\end{tabular}}}}  & \multicolumn{1}{c|}{\multirow{8}{*}{\textbf{Shallow}}} & \multirow{8}{*}{SHS} & \multicolumn{1}{c|}{\multirow{2}{*}{Random}} & Min Tiles             & 10             & 1             & 10            & Compact             & 15-to-1                                      & 19               & 11              & 31               \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 10             & 1             & 10            & Fast                & 20-to-4                                      & 18               & 17              & 34               \\ \cline{4-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{\multirow{2}{*}{BF}}     & Min Tiles             & 10             & 1             & 10            & compact             & 15-to-1                                      & 11               & 3               & 29               \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 10             & 1             & 10            & fast                & 15-to-1 ; 225-to-1                           & 11               & 10              & 216              \\ \cline{4-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{\multirow{2}{*}{DP}}     & Min Tiles             & 10             & 1             & 10            & compact             & 15-to-1                                      & 11               & 3               & 29               \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 10             & 1             & 10            & fast                & 15-to-1 ; 20-to-4                            & 11               & 10              & 54               \\ \cline{4-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{\multirow{2}{*}{Greedy}} & Min Tiles             & 10             & 1             & 10            & compact             & 20-to-4 (2)                                  & 25               & 17              & 46               \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 10             & 1             & 10            & fast                & 20-to-4 (2)                                  & 18               & 17              & 57               \\ \cline{2-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{\multirow{8}{*}{\textbf{Deep}}}    & \multirow{8}{*}{DLL} & \multicolumn{1}{c|}{\multirow{2}{*}{Random}} & Min Tiles             & 100            & 5833          & 5833          & Compact             & 15-to-1                                      & 64171            & 40550           & 211              \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 100            & 5833          & 5833          & Fast                & 20-to-4                                      & 24804            & 21085           & 214              \\ \cline{4-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{\multirow{2}{*}{BF}}     & Min Tiles             & 100            & 5833          & 5833          & compact             & 15-to-1                                      & 40524            & 17247           & 164              \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 100            & 5833          & 5833          & fast                & 15-to-1 ; 116-to-12 ; 225-to-1 (2);  20-to-4 & 7185             & 3501            & 649              \\ \cline{4-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{\multirow{2}{*}{DP}}     & Min Tiles             & 100            & 5833          & 5833          & compact             & 15-to-1                                      & 40656            & 17133           & 164              \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 100            & 5833          & 5833          & fast                & 15-to-1 ;  20-to-4 (2)                       & 11340            & 7644            & 267              \\ \cline{4-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{\multirow{2}{*}{Greedy}} & Min Tiles             & 100            & 5833          & 5833          & compact             & 20-to-4 (2)                                  & 23245            & 17              & 181              \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 100            & 5833          & 5833          & fast                & 20-to-4 (2)                                  & 11324            & 7645            & 256              \\ \hline \hline
\multicolumn{1}{c|}{\multirow{16}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}T Gate\\ Density\end{tabular}}}} & \multicolumn{1}{c|}{\multirow{8}{*}{\textbf{Low}}}     & \multirow{8}{*}{SLS} & \multicolumn{1}{c|}{\multirow{2}{*}{Random}} & Min Tiles             & 30             & 625           & 4401          & Compact             & 15-to-1                                      & 6883             & 2015            & 71               \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 30             & 625           & 4401          & Fast                & 20-to-4                                      & 2670             & 2045            & 74               \\ \cline{4-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{\multirow{2}{*}{BF}}     & Min Tiles             & 30             & 625           & 4401          & compact             & 15-to-1                                      & 6875             & 2043            & 59               \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 30             & 625           & 4401          & fast                & 20-to-4 (2)                                  & 1201             & 576             & 103              \\ \cline{4-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{\multirow{2}{*}{DP}}     & Min Tiles             & 30             & 625           & 4401          & compact             & 15-to-1                                      & 6875             & 2055            & 59               \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 30             & 625           & 4401          & fast                & 15-to-1 ;  20-to-4 (2)                       & 1923             & 1298            & 114              \\ \cline{4-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{\multirow{2}{*}{Greedy}} & Min Tiles             & 30             & 625           & 4401          & compact             & 20-to-4 (2)                                  & 4855             & 17              & 76               \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 30             & 625           & 4401          & fast                & 20-to-4 (2)                                  & 1201             & 576             & 103              \\ \cline{2-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{\multirow{8}{*}{\textbf{High}}}    & \multirow{8}{*}{SHM} & \multicolumn{1}{c|}{\multirow{2}{*}{Random}} & Min Tiles             & 50             & 417           & 15741         & Compact             & 15-to-1                                      & 4595             & 1259            & 111              \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 50             & 417           & 15741         & Fast                & 20-to-4                                      & 1786             & 1369            & 114              \\ \cline{4-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{\multirow{2}{*}{BF}}     & Min Tiles             & 50             & 417           & 15741         & compact             & 15-to-1                                      & 4587             & 1251            & 89               \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 50             & 417           & 15741         & fast                & 20-to-4 (2)                                  & 800              & 383             & 148              \\ \cline{4-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{\multirow{2}{*}{DP}}     & Min Tiles             & 50             & 417           & 15741         & compact             & 15-to-1                                      & 4587             & 1251            & 89               \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 50             & 417           & 15741         & fast                & 15-to-1 ;  20-to-4 (2)                       & 1287             & 870             & 159              \\ \cline{5-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{\multirow{2}{*}{Greedy}} & Min Tiles             & 50             & 417           & 15741         & compact             & 20-to-4 (2)                                  & 3353             & 17              & 106              \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 50             & 417           & 15741         & fast                & 20-to-4 (2)                                  & 800              & 383             & 148              \\ \hline \hline
\multicolumn{1}{c|}{\multirow{16}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Qubit\\ Count\end{tabular}}}}    & \multicolumn{1}{c|}{\multirow{8}{*}{\textbf{Small}}}   & \multirow{8}{*}{MHS} & \multicolumn{1}{c|}{\multirow{2}{*}{Random}} & Min Tiles             & 20             & 1333          & 21383         & Compact             & 15-to-1                                      & 14671            & 4003            & 51               \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 20             & 1333          & 21383         & Fast                & 20-to-4                                      & 5679             & 4346            & 54               \\ \cline{4-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{\multirow{2}{*}{BF}}     & Min Tiles             & 20             & 1333          & 21383         & compact             & 15-to-1                                      & 14663            & 3991            & 44               \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 20             & 1333          & 21383         & fast                & 20-to-4 (2)                                  & 2581             & 1248            & 80               \\ \cline{4-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{\multirow{2}{*}{DP}}     & Min Tiles             & 20             & 1333          & 21383         & compact             & 15-to-1                                      & 14663            & 3997            & 44               \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 20             & 1333          & 21383         & fast                & 15-to-1 ;  20-to-4 (2)                       & 4097             & 2764            & 91               \\ \cline{4-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{\multirow{2}{*}{Greedy}} & Min Tiles             & 20             & 1333          & 21383         & compact             & 20-to-4 (2)                                  & 10684            & 17              & 61               \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 20             & 1333          & 21383         & fast                & 20-to-4 (2)                                  & 2581             & 1248            & 80               \\ \cline{2-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{\multirow{8}{*}{\textbf{Large}}}   & \multirow{8}{*}{MML} & \multicolumn{1}{c|}{\multirow{2}{*}{Random}} & Min Tiles             & 90             & 3000          & 103125        & Compact             & 15-to-1                                      & 33008            & 9008            & 191              \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 90             & 3000          & 103125        & Fast                & 20-to-4                                      & 12754            & 9754            & 194              \\ \cline{4-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{\multirow{2}{*}{BF}}     & Min Tiles             & 90             & 3000          & 103125        & compact             & 15-to-1                                      & 33000            & 9000            & 149              \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 90             & 3000          & 103125        & fast                & 20-to-4 (2)                                  & 5831             & 2831            & 234              \\ \cline{4-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{\multirow{2}{*}{DP}}     & Min Tiles             & 90             & 3000          & 103125        & compact             & 15-to-1                                      & 33000            & 9000            & 149              \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 90             & 3000          & 103125        & fast                & 15-to-1 ;  20-to-4 (2)                       & 9200             & 6200            & 245              \\ \cline{4-13} 
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{\multirow{2}{*}{Greedy}} & Min Tiles             & 90             & 3000          & 103125        & compact             & 20-to-4 (2)                                  & 24017            & 17              & 166              \\
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                  &                      & \multicolumn{1}{c|}{}                        & Min Steps             & 90             & 3000          & 103125        & fast                & 20-to-4 (2)                                  & 5831             & 2831            & 234              \\ \hline \hline
\end{tabular}
\end{adjustbox}
\label{tab:big_table}
\end{table*}
